AutoAlign: Pixel-Instance Feature Aggregation for Multi-Modal 3D Object Detection

Object detection through either RGB images or the LiDAR point clouds has been extensively explored in autonomous driving. However, it remains challenging to make these two data sources complementary and beneficial to each other. In this paper, we propose \textit{AutoAlign}, an automatic feature fusion strategy for 3D object detection. Instead of establishing deterministic correspondence with camera projection matrix, we model the mapping relationship between the image and point clouds with a learnable alignment map. This map enables our model to automate the alignment of non-homogenous features in a dynamic and data-driven manner. Specifically, a cross-attention feature alignment module is devised to adaptively aggregate \textit{pixel-level} image features for each voxel. To enhance the semantic consistency during feature alignment, we also design a self-supervised cross-modal feature interaction module, through which the model can learn feature aggregation with \textit{instance-level} feature guidance. Extensive experimental results show that our approach can lead to 2.3 mAP and 7.0 mAP improvements on the KITTI and nuScenes datasets, respectively. Notably, our best model reaches 70.9 NDS on the nuScenes testing leaderboard, achieving competitive performance among various state-of-the-arts.

==> tables/kitti.tex <==
\begin{table}[!b]
		\centering
		\begin{threeparttable}
			\begin{tabular}{c | c c c}
				\toprule
				\multirow{2}*{Query Method}  &    & $\text{AP}_{3D}$(\%) & \\
				   & Easy & Mod. & Hard\\
				 \midrule
				 Point-based Proj & 80.24 & 69.40 & 65.65\\
				 Non-Local & 80.01 & 69.13 & 65.34\\
				 Multi-head Cross-attention & 81.04 & 70.25 & \textbf{66.49}\\
				 Single head Cross-attention & \textbf{81.29} & \textbf{70.31} & 66.44\\
				\bottomrule
			\end{tabular}
		\end{threeparttable}
		\caption{$\text{AP}_{3D}$ performance with various query methods for cross-modality feature alignment.}
	\label{tab:ablation_query}
\end{table}

==> tables/kitti_sota.tex <==
\begin{table*}[!h]
	\centering
		\begin{threeparttable}
		\setlength{\tabcolsep}{1.6mm}
			\begin{tabular}{c | c c c | c c c | c c c | c c c }
				\toprule
				\multirow{2}*{Method}  &  \multicolumn{3}{c|}{Car $\text{AP}_{3D}$ (\%)} & \multicolumn{3}{c|}{Pedestrian $\text{AP}_{3D}$ (\%)} & \multicolumn{3}{c|}{Cyclist $\text{AP}_{3D}$ (\%)} & \multicolumn{3}{c}{Overall $\text{AP}_{3D}$ (\%)}\\
				     & Easy & Mod. & Hard & Easy & Mod. & Hard & Easy & Mod. & Hard & Easy & Mod. & Hard\\
				\midrule
				AVOD-FPN \cite{ku2018joint} & 83.1 & 71.8 & 65.7 & 50.5 & 42.3 & 39.0 & 63.8 & 50.6 & 44.9 & 65.8 & 54.9 & 49.9\\
				F-PointNet \cite{qi2018frustum}  & 82.2 & 69.8 & 60.6 & 50.5 & 42.2 & 38.1 & 72.3 & 56.1 & 49.0 & 68.3 & 56.0 & 49.2\\
				PointPainting \cite{vora2020pointpainting}  & 82.1 & 71.7 & 67.0 & 50.3 & 41.0 & 37.9 & 77.6 & 63.8 & 55.9 & 70.0 & 58.8 & 53.6 \\
				MoCa \cite{zhang2020exploring}  & 86.0 & 75.9 & 70.7 & 50.9 & 43.7 & 40.0 & 76.1 & 61.0 & 53.4 & 71.0 & 60.2 & 54.7\\
				\midrule
				AutoAlign (Ours) & \textbf{86.8} & \textbf{77.6} & \textbf{73.2} & \textbf{54.0} & \textbf{44.1} & \textbf{40.8} & \textbf{80.4} & \textbf{64.4} & \textbf{56.9} & \textbf{73.7} & \textbf{62.1} & \textbf{57.0}\\
				\bottomrule
			\end{tabular}
		\end{threeparttable}
		\caption{Comparison with state-of-the-art multi-modal 3D detectors on KITTI 3D testing benchmark.}
	\label{tab:kitti_sota}
%	\vskip -0.5em
\end{table*}

==> tables/waymo.tex <==
\begin{table*}[hbpt]
    \centering
    \label{tab::waymores}
    \setlength{\tabcolsep}{1.6mm}
    \begin{tabular}{c | c|cc|cc|cc|cc}
    \toprule
    \multirow{2}{*}{Method} &
    \multirow{2}{*}{AutoAlign} &
    \multicolumn{2}{c|}{Vehicle L1/L2} &
    \multicolumn{2}{c|}{Pedestrian L1/L2} &
    \multicolumn{2}{c|}{Cyclist L1/L2} &
    \multicolumn{2}{c}{Mean L1/L2} \\
       &  & AP & APH & AP & APH & AP & APH & AP & APH\\     
	\midrule
   	\multirow{2}*{PointPillar} & & 61.1/57.3 & 60.7/56.8 & 60.8/55.7 & 46.4/43.0 & 60.2/57.8 & 57.7/55.3 & 60.7/56.9 & 54.9/51.5 \\
      & \checkmark & \textbf{62.2/58.4} & \textbf{61.8/57.7} & \textbf{61.2/55.9} & \textbf{46.7/43.5} & \textbf{63.1/60.5} & \textbf{60.7/58.3} & \textbf{62.1/58.2} & \textbf{56.4/53.1}\\
    \midrule
    \multirow{2}*{SECOND} &  & 64.4/61.1 & 63.7/60.5 & 66.6/61.9 & 57.5/53.0 & 61.2/58.6 & 58.3/55.7 & 64.0/60.5 & 59.8/56.4\\
      & \checkmark & \textbf{66.5/62.4} & \textbf{66.0/61.9} & \textbf{67.6/62.9} & \textbf{58.7/53.9} & \textbf{64.2/61.5} & \textbf{61.2/58.7} & \textbf{66.1/62.3} & \textbf{62.0/58.2}\\
    \bottomrule
    \end{tabular}
    \caption{AP performance on different 3D object detectors w/o and w/ AutoAlign on WOD validation set.}
    \label{tab:waymo_all}
    \vskip -0.5em
\end{table*}

==> tables/waymo_dis.tex <==
\begin{table*}[!hbpt]
    \centering
    \label{tab::waymores}
    \setlength{\tabcolsep}{1.6mm}
    \begin{tabular}{c | c | c|ccc|c|ccc}
    \toprule
    \multirow{2}{*}{Method} &
    \multirow{2}{*}{AutoAlign} &
    \multicolumn{4}{c|}{Vehicle L1/L2} &
    \multicolumn{4}{c}{Pedestrian L1/L2} \\
       &  & Overall & 0-30m & 30-50m & 50m-Inf & Overall & 0-30m & 30-50m & 50m-Inf \\     
	\midrule
	\multirow{2}*{SECOND} & & 64.4/61.1 & 86.3/86.1 & 68.1/66.7 & 46.3/40.5 & 66.6/61.9 & 75.6/74.9 & 68.4/65.5 & 57.0/49.9 \\
		& \checkmark & 66.5/62.4 & 87.3/87.1 & 68.9/67.5 & 48.2/42.7 & 67.6/62.9 & 76.3/75.6 & 68.8/65.2 & 60.1/53.0\\
	\midrule
%		\rowcolor{green}\multicolumn{2}{c|}{improvement} & +2.1/+1.3 & + 1.0/+1.0 & +0.8/+0.8 & +1.9/+2.2 & +1.0/+1.0 & +0.7/+0.7 & +0.4/-0.3 & +3.1/+3.1\\
		\multicolumn{2}{c|}{Improvement} & \textbf{+2.1/+1.3} & +1.0/+1.0 & +0.8/+0.8 & \textbf{+1.9/+2.2} & \textbf{+1.0/+1.0} & +0.7/+0.7 & +0.4/-0.3 & \textbf{+3.1/+3.1}\\
    \bottomrule
    \end{tabular}
    \caption{AP performance under different distance-based evaluation protocol on WOD validation set.}
    \label{tab:waymo_dist}
    \vskip -0.1em
\end{table*}
